Multi-Layer Personalized Federated Learning for Mitigating Biases in Student Predictive Analytics

Conventional methods for student modeling, which involve predicting grades based on measured activities, struggle to provide accurate results for minority/underrepresented student groups due to data availability biases. In this paper, we propose a Multi-Layer Personalized Federated Learning (MLPFL) methodology that optimizes inference accuracy over different layers of student grouping criteria, such as by course and by demographic subgroups within each course. In our approach, personalized models for individual student subgroups are derived from a global model, which is trained in a distributed fashion via meta-gradient updates that account for subgroup heterogeneity while preserving modeling commonalities that exist across the full dataset. The evaluation of the proposed methodology considers case studies of two popular downstream student modeling tasks, knowledge tracing and outcome prediction, which leverage multiple modalities of student behavior (e.g., visits to lecture videos and participation on forums) in model training. Experiments on three real-world online course datasets show significant improvements achieved by our approach over existing student modeling benchmarks, as evidenced by an increased average prediction quality and decreased variance across different student subgroups. Visual analysis of the resulting students' knowledge state embeddings confirm that our personalization methodology extracts activity patterns clustered into different student subgroups, consistent with the performance enhancements we obtain over the baselines.

==> tables/TKDE_sc1_ktpp_improve.tex <==

\begin{table}[tp]
\caption{\color{blue}AUC improvement from the population-level method \texttt{[sc1-G]} for knowledge tracing (KT) and outcome prediction (OP) across different models in the MOSFETs course. \color{black}}

\begin{center}

\scalebox{0.9}{

\begin{tabular}{ccc}
\hline
\multicolumn{1}{c}{Model} & KT & OP \\ \hline\hline
\texttt{[sc1-G-AV]} & $-$.002& $-$.002  \\
\texttt{[sc1-G-AT]} & $-$.012  & $-$.005  \\
 \texttt{[sc1-P-AV]} & $+$.072 & $+$.105 \\
\texttt{[sc1-P-AT]}(MLPFL) & \textbf{$+$.088}& \textbf{$+$.126} \\
\hline
\end{tabular}
}
\end{center}
\vspace{-0.25in}

\label{tb:sc1_improve}
\end{table}

==> tables/TKDE_sc2_kt_improve.tex <==

\begin{table*}[htp]
\caption{\color{blue}AUC improvement over the population-level method \texttt{[sc2-G]} for the outcome prediction task across different personalized models for each minority group in each course.
 \color{black}}

\begin{center}

\scalebox{0.9}{

\begin{tabular}{lcccccccccc}
\hline
\multicolumn{1}{c|}{Dataset}& \multicolumn{3}{c|}{FOC} & \multicolumn{3}{c|}{QDS}  & \multicolumn{3}{c}{MOSFETs}\\  \hline
\multicolumn{1}{c|}{Model} & female & AS & \multicolumn{1}{c|}{$<80$} & female & AS & \multicolumn{1}{c|}{$<80$} & female & AS & $<80$ \\
\hline
\texttt{FedIRT} & $+$.026 & $+$.099 & $+$.104 & $+$.010 & $+$.065 & $+$.047 & $+$.022 & $-$.039 & $+$.026\\
\texttt{[sc2-P-AV-M]} & $+$.093 & $+$.000 & $+$.087 & $+$.076 & $+$.066 & $+$.024 & $+$.031 & $-$.036 & $+$.064\\
\texttt{[sc2-P-AT-M]}(MLPFL) & $+$.111 & $+$.050 & $+$.099 & $+$.102 & $+$.139 & $+$.047 & $+$.027 & $-$.023 & $+$.070\\
\texttt{[sc2-P-AV-B]} & $+$.133 & $+$.097 & $+$.133 & $+$.112 & $+$.141 & $+$.080 & $+$.082 & $+$.017 & \textbf{$+$.108}\\
\texttt{[sc2-P-AT-B]}(MLPFL)& \textbf{$+$.140} & \textbf{$+$.116} &\textbf{ $+$.145} & \textbf{$+$.115} & \textbf{$+$.156} & \textbf{$+$.096} & \textbf{$+$.100} & \textbf{$+$.031} & $+$.106 \\
\hline



\end{tabular}
}
\end{center}
% \vspace{-0.1in}
% \vspace{-0.3in}
\vspace{-0.2in}

\label{tb:sc2_improve}
\end{table*}
